Affective Learning Objectives for Communicative Visualizations

When designing communicative visualizations, we often focus on goals that seek to convey patterns, relations, or comparisons (cognitive learning objectives). We pay less attention to affective intents--those that seek to influence or leverage the audience's opinions, attitudes, or values in some way. Affective objectives may range in outcomes from making the viewer care about the subject, strengthening a stance on an opinion, or leading them to take further action. Because such goals are often considered a violation of perceived 'neutrality' or are 'political,' designers may resist or be unable to describe these intents, let alone formalize them as learning objectives. While there are notable exceptions--such as advocacy visualizations or persuasive cartography--we find that visualization designers rarely acknowledge or formalize affective objectives. Through interviews with visualization designers, we expand on prior work on using learning objectives as a framework for describing and assessing communicative intent. Specifically, we extend and revise the framework to include a set of affective learning objectives. This structured taxonomy can help designers identify and declare their goals and compare and assess designs in a more principled way. Additionally, the taxonomy can enable external critique and analysis of visualizations. We illustrate the use of the taxonomy with a critical analysis of an affective visualization.

==> 99_assessments.tex <==
\section{Assessment}

An application of how assessments could look like for affective learning objectives.

\subsection{Multiple Choice Questions}
-pre and -post design

Likert questions

Scott and Wheeless, 1977
Seven interval scales 
Attitudes on good/bad, worthless/valuable, fair/unfair, and positive/negative

Kurdi, Lozano, \& Banaji, 2017
Measured valence (negative to positive) and arousal (low to high)

Pandey et. al., 2014 
The “two main established methods” are the bipolar adjectives and the single-item scales, they went with the latter. -> “To what extent do you agree that lowering the federal corporate in- come tax rate creates jobs?” from +3 to -3

Nell Buissink-Smith, Samuel Mann and Kerry Shephard, 2011
Several dimensions discussed: short vs long term, primary vs secondary sources, quantitative vs qualitative. A lot of the specific examples were validated questionnaires about environmental attitudes.
Quantitative:
self-reporting
pre and post tests
Likert scales
bipolar adjectives
Thurstone equal appearing interval scale
importance-performance analysis
forced choice
Q methodology

Multiple items:
Itzchakov 2018
Self-control depletion increases persuasion but not behavior
Participants rated their attitude towards veganism on six items ranging from 1 = strongly disagree to 9 = strongly agree (“veganism is a good thing”, “I'm in favor of veganism”, “veganism is a desired thing”, “veganism is a negative thing”, “veganism is silly”, “veganism is a useful thing”), $\alpha$ = 0.94.


\subsection{Qualitative Methods}

Nell Buissink-Smith, Samuel Mann and Kerry Shephard, 2011
Several dimensions discussed: short vs long term, primary vs secondary sources, quantitative vs qualitative. A lot of the specific examples were validated questionnaires about environmental attitudes.
Qualitative:
Observations
Focus groups
Interview
Reflective journaling
Videos, games
Drawings
Personal mapping meaning
Actions
Think aloud


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> thoughts.tex <==
%% This file is thoughts written out about a few topics that will eventually be brought into the actual first draft of the paper

\subsection{Neutral intents}

What do we really mean by "neutral" intents? Perhaps we mean "non-political" or "trustworthy"? 

On the Vox video, they commented that Portugal's strategy was "to give the vaccine effort a non-political face", which resulted in a 91\% rate of the population getting a vaccine. Compared to the US's 64\% rate. Is it possible to have something be non-political in the United States? Portugal's strategy was to use the military for messaging. The officer's look and demeanor(?) gives off both an air of authority and trustworthiness. To me, the objective is - The viewer will get vaccinated. Here, political "neutrality" might be a technique/method/strategy to achieve their goal. A design decision. Could there be a learning objective there? The viewer will perceive the vaccination campaign as non-political. I'm not sure how that fits. 

Maybe the strategy could be really helpful as an affective learning objective - to get the designer thinking about the audiences' prior knowledge, beliefs, and attitudes, and to think about what sort of message would be most effective to reach those people. This makes me think back to Kat's discussion of climate change in her interview. 

Vox's comment was interesting - they were wondering whether a military-led approach would have reduced polarization in the US. I believe the attitudes toward the military are conservative - leaning. So it's already polarized in that way potentially. However, this could have actually been helpful, as potentially conservatives are the ones that are reluctant to get the vaccine. So more liberal people could be brought on board with vaccination and public health, conservative people could be brought on board with the military and America first America best messaging. It's very sad to hear in the Vox video about the public's lack of trust of authority/media/CDC.

Overall here, I think it's worthwhile to be more specific about what people mean when they have a goal of "objectivity" or "neutrality". - "non-partisan" "trustworthy" etc? What are some more examples? "scientific" "transparent" "understandable" 

I wonder how this intersects with Cole Nussbaumer Knafflic's idea of Focusing the graph by putting the main message as the title. Is it possible to have a Focused graph that also is "neutral"? How much is this influenced by topic of the data?

\subsection{Thoughts on BC Interview}

So people who have been doing data visualization for a significant amount of time might have a solid and set process that they use. But on the other hand it also seems like the people who are most likely to have an affective intent are people who have been working with data visualization on more of an advanced level.

Are women and people of color more likely to have affective visualizations?

White men: 3
White women: 5 
Non-white men: 1 
Non-white women: 1 

Hmm, but this does not answer that question. Maybe white people and women make up a higher proportion of the DVS population? Maybe 6-4 is not significantly different. Maybe white women are more likely to share in the #share-showcase and #share-critique channels. 

\subsection{Journalism and Impartiality}

From the Society of Professional Journalists: 
    Seek Truth and Report It
    – Label advocacy and commentary. 
    Act Independently
    – Refuse gifts, favors, fees, free travel and special treatment, and avoid political and other outside activities that may compromise integrity or impartiality, or may damage credibility. 
    https://www.spj.org/ethicscode.asp

American Press Association
    Independence is an underlying requirement of journalism, a cornerstone of its reliability. Independence of spirit and mind, rather than neutrality, is the principle journalists must keep in focus. 
    https://americanpressassociation.com/principles-of-journalism/
    
NPR
    The impartiality extends to the journalists' personal lives, restrictions on what they can do / say in order to not seem to have any biases that could potentially be reflected in their writing. 
    QUOTE: "A large part of what makes our work so valuable is our effort to transcend how we feel about a subject and impart to our audience what we know about it, and what we don't."
    Section about commentary, criticisms, essays
    Neutral language choices
    https://www.npr.org/about-npr/688413430/impartiality
    
BBC    
   Due Impartiality
   https://www.bbc.co.uk/editorialguidelines/guidelines/impartiality
   
OfCom
    https://www.ofcom.org.uk/tv-radio-and-on-demand/broadcast-codes/broadcast-code/section-five-due-impartiality-accuracy
    
Due Impartiality - Climate Change no longer has to give any airtime to deniers. Human rights issues are things to support. Trans rights are still up for debate.
    https://www.theguardian.com/media/2021/nov/12/what-does-impartiality-mean-bbc-no-bias-policy-being-pushed-to-limits
    
NPR examples of the same topic as news and opinion
https://www.npr.org/2019/12/20/790319846/why-author-j-k-rowling-is-facing-backlash-from-lgbtq-activists
https://www.npr.org/2020/06/10/873472683/harry-potters-magic-fades-when-his-creator-tweets

Also reminds me of this twitter bot: %https://twitter.com/nyt_diff?lang=en

\subsection{Part of an Outline}

Points that we should potentially make (& cite) in this paper:
  - Some people (journalists) claim to purely inform / be neutral or impartial
      BUT
      - Data is not neutral (VIS capstone, Correll ethics, Data Feminism)
      - Visualizations are not neutral (Correll ethics, Rhetorical Hullman & Diakopolous)
      - Visualizations can be used for persuasive intents besides what the author intended
  - People could be unaware of their biases and unintentionally put a persuasive spin on it
  - People could have ill intents and persuade for bad reasons (Black hat visualization)
  ALSO
  - People create visualizations with affective intents on purpose - i.e. advocacy
  THEREFORE
  - This taxonomy can help people with affective intents be more aware of them and create more effective visualizations
     - This taxonomy can make unaware people aware of their persuasive intents/biases
  - This taxonomy can be used to critique/judge other peoples' (ill) intents
  - This taxonomy can help you articulate anti-objectives ? for neutrality ? 
        - Neutrality - Politically balanced, minority opinions
        - Neutrality - No emotional trigger

Decisions to not show visualizations are also political
Would people be willing to use the taxonomy?
Feeling challenged by self-reflection
Consumerism Advertising

\section{Reversing the Abstraction}

Humanizing the data 

\section{Discomfort with Designer's Power}

\section{Reflection on IdlT Interview}

Irene was nice. It was interesting to hear her struggles with the direction of the visualization changing over time within the collaboration of her news team. I wonder if having learning objectives would have helped them all communicate with each other on the direction and purpose of the visualization.

\section{Reflection on VB Interview}

Well this interview I did was kind of hard to follow. It sounded like this participant didn't quite have the grasp on affective intents like some of my other participants did. He sort of went off topic a few times. And then at the end did like a huge ramble on about his creative coding class... so. Not the most focused interview. I did try to dig in and get a little bit deeper of an understanding of what he was saying, but I'm not really sure if I got that far. 

It is interesting when participants don't really have a framework for how they do think about intent. I feel like people learn by making connections to what they already know (shoutout to Kevin Miller). So when people already have an idea of how they conceptualize or think about communicative intent in their design process, it's easier for them to learn about learning objectives. It maybe makes it easier for them to imagine themselves integrating it into their own design process. The hard part is that everyone's design process and conceptualization of communicative intent is different... so it doesn't integrate the same way for everyone. 

There was a bit where Ed was talking about shouting is destroying the message, which is I think getting more into the design of the visualization rather than the goals of the visualization. Was he conflating the two? It was not always very clear about what he was talking about. He talks about his audience being an informed audience that already believes what he talks about, then talks about journalists too.

The part about accidental learning objectives or hidden learning objectives makes me think that he didn't quite understand learning objectives. Learning objectives are the intentional goals that a teacher/designer has. Any unintended consequence of the data visualization is not an objective. It may be an outcome, but not an objective. The part about having "hidden learning objectives" or lying with statistics or the data or ignoring the actual data and having your own agenda... these are all interesting things about data visualization... but I'm not sure how much they actually relate to this learning objectives study. Maybe it does. Maybe it's very much related to being aware of your biases and being aware of other people's biases. For example, that data visualization put out by the Biden administration on the strongest economy year since the 80s or whatever. It crops the x axis time to start at the year 2000. When you include more of the data from the 80s to now, the message of the graph isn't as strong, because the 90s had a strong economy or something. The designers of the graph probably had an objective to show how good Biden is doing. Was it such a crime to start the X axis at the year 2000? Maybe, because the point was that it's the highest since the 80s. 

It was pretty cool to have two people discussing the learning objectives. It sort of shows how it could be used as a communication social object device to facilitate better discussion of goals. 


\section{SJ Interview (from last study)}

"I wanted to just maybe come up with articles which are totally fact-based, totally data driven, not opinionated, and just putting data out there in a way that you can understand and grasp quickly. "

"when setting up the project I want to communicate that this is the objective behind my project, and I think, I believe I would want people to have their own takeaways, even though I have a particular idea in mind that this is what they should get out of the project. "

\section{Reflection on JS Interview}

Where does the power lie in the relationship between the designer and the reader in the communication of the data visualization?

Some designers feel uncomfortable with the idea that their work will influence, persuade, or have a hand in changing their audience's opinions, beliefs, or values. 

An author, creator, or designer of a visualization has the power of unilaterally making design decisions of how the visualization will turn out. As argued in our previous paper [cite], designers have the option to, and often do, take into consideration the characteristics and goals of their audience. However, the audience does not get a say in what the designer ultimately chooses to be the visualization. 

On the other hand, for a data practitioner putting their work out into the ether, they often don't have control over forcing people to view their work. In the case of data journalism, the authors create content for the subscribers or readers of the platform, but they have no control over whether the readers will actually read or engage with their piece. This is akin to the designer being in the role of a "radio host" [cite MS], where they get to choose which channel to tune into and which channel to turn down the volume on. Even though the reader has this choice in what to listen to, the designer has the platform, reach, and power of their position to disseminate information. 

Taken out of context

Of course, this varies by position. If you are a senior data journalist at a popular newspaper, that position comes with a great power and great responsibility. On the other hand, a hobbyist who creates data visualization for fun might not have an audience. Even so, the hobbyist has a responsibility to work with data ethically, responsibly, and truthfully. 

Participant JS works on open source data visualization projects as a hobby. He created a visualization that represented the finite length of a person's life. He describes an ideal response to his visualization as the viewer would consider the finity of life and modify their habits to be more productive. However, he was very reluctant to agree that his goal was that the viewer would change their behavior. He wanted to hinge that goal on the condition that it was really up to the viewer about whether or not they would actually change their behavior. 

In one way, it will always depend on the viewer on whether or not the visualization will be effective in achieving the designer's goal. On the other hand, it is unfaithful/not in good faith/misrepresenting/lying/untruthful for the designer to not admit that their goal is to change the viewer's behavior. Whether or not the designer admits it or externalizes it, all designers have biases and their own goals of what they want the viewer to do or know after viewing their data visualization. 

The cognitive aspect of communicating information is straightforward, uncontroversial, and largely agreed upon by the data visualization community. Affective goals are the opposite. Persuasion, emotion, and influencing an audience's beliefs or values is of large debate in this community. 



\section{Reflection on MS Interview}

MS actually participated in the first interview study on learning objectives so it was nice to see him again! Because of this, one thing that I was interested in was asking if he did use learning objectives since our last conversation, and it seems like the answer was "No" but that he did take away one concept of "What will the viewer take away or know after (like tomorrow) they see my visualization". Which is kind of nice! It was also very fun to hear how his career has taken off in the past two years. 

When I first introduced the concept of Affective Learning Objectives, the first thing that he thought of was that they were more abstract and long-term. Which, I guess opinions and values are kind of more abstract than facts, but I did try to give examples of long-term cognitive learning objectives as well. 

Something interesting is that he mentioned 100,000 as a very large number that is hard to understand the magnitude of. This is something that JWT also talked about, but in a different way sort of. 

Cognitive learning objectives:
1. The viewer will explain the scrollytelling technique.
2. The viewer will check the facts of the 2nd wave of coronavirus. 

Affective learning objectives:
1. The viewer will modify their opinions
- COVID is/will not hit me
- There are only a few -> many people dying from COVID
2. The viewer will trust the data
3. (Secret objective) The politician will be influenced.

Overall, MS was maybe not the best at creating learning objectives. He seemed to struggle and he did report that it was difficult. A successful comment would be one that expressed sad emotions... and something else.

He seemed to need to have different learning objectives for different audiences.

The learning objectives would be most useful for larger projected that involved creativity and novel data visualization formats.

Evoking emotions is the method.

One piece of inspiration was this piece that MS worked on for a different project: http://billshander.com/dataviz/trumps-year-of-covid/
I think it's interesting how there's intstructions on how they want you to experience the visualization. I definitely think that MS's version is an improvement. They both had different goals though. 

MS's visualization: Here are some aspects that I loved.
1. Each person is a dot
2. Dot is big so you can see it and then small so you can really see them accumulate
3. Animation
4. Dark mode
5. Interactivity with scrollytelling
6. Images!
7. Text for storytelling

What's interesting about his design process is that he's had these ideas from inspiration and previous work. Just having ideas and seeing what works. Not looking into the data vis literature or anything formal. 

Very cool. Also I probably could have talked to him longer about psychic numbing. Anyways he also declined compensation for his time. 

\section{Reflection on GM Interview}

So far, everyone (2/2) that I've interviewed has understood what I've meant by learning objectives. One potential reason for this is that trying to evoke an affective response from an audience is sort of a "next-level" or more advanced goal of creating a data visualization. Potentially, people who have these sort of goals are already thinking more about their audience and the effect that their visualization will have on their audience, and therefore they are more amenable to these conversations and ideas. 

Even though GM "totally" understood learning objectives, she still did not get the fact that the learning objective would be something that the reader would do *after* they viewed the visualization. Obviously, I did not explain this at all, and should consider putting it in the powerpoint. I want to go back and re-listen to the part of the interview where she talks about emotion. That's pretty interesting to me, thinking about how emotion plays a role in this. 

It is interesting that her "ideal" social media response would be to share the post, although now that I'm writing this down, I'm realizing that maybe she was constraining herself to the three options of "like, comment, share". But, to "share" in her mind was to indicate that the reader had learned something new. In this case, she was trying to correct a misconception that China and India are the most responsible for carbon emissions. 

One other interesting tidbit is that she calls these "data illustrations" which are similar and close to "data art", but are a little bit closer to the data side than the purely art side.

\section{Thoughts on the first Interview}

Some participants struggled with understanding and creating learning objectives. However, some participants understood learning objectives without any problem, and were immediately able to create learning objectives of their own. 

Furthermore, we identified a need for more resources to provide to data visualization practitioners to enable them to create learning objectives in their design process. X participants indicated that learning objectives were useful and they intended on using them in a future project. X participants indicated that learning objectives were [XYZ] and that they would probably be not using them again. For the reluctant designers, we agree that learning how to create learning objectives has a learning curve. However, more in depth instructional materials may help bridge this gap to making specifying communicative intent more helpful than it is onerous. 

\section{Thoughts on the panel "Visualizing Climate Change"}

One interesting thing from this panel discussion was that the journalists on the call saw their goal as to inform rather than persuade. One person also mentioned a goal that was to “evoke curiosity” which Alberto Cairo also saw as an emotion goal. Although Alberto was discussing ways that data visualization could bring emotion and visceralize the data, he stated that he was skeptical of the persuasive power of data visualization and that he thought that it would be useful to pair data vis with other techniques from domains such as gaming, cinema, and writing. He saw data visualization as an analytical tool, that was designed for analytical tasks. He mentioned the plastic water bottles and said that the visual imagery was really striking. Data visualization can be very abstract and having these visual images and pictoral images can help. 

One thing that more than one person mentioned was personalizing the visualization to be proximally relevant to the viewer’s location. 

One very interesting thing that Alberto Cairo said was that people don’t trust numbers alone. Having a narrator like Hans Rosling explain the data could help. 

Another interesting thing was that the industries don’t usually evaluate their graphs on their intended audience. It’s not necessary for a simple bar chart or line chart. But for more complicated graphs, they don’t do it either. The daily graphic did do some user testing when it first launched and learned that they needed to do more simple charts. 

A goal to have the visualization be a conversation starter! The #showyourstripes vis breaks all the conventional data visualization rules - no axes or labels! But it WORKS because people love it and people want to talk about it. It’s a simple graph, it’s a visually appealing graph, and it’s personalized to the viewer’s location. It’s also quite intuitive as people generally connect the temperature representation to the color encoding. 



\section{The nouns of the taxonomy}

\section{Data art}

\section{The goal of a conversation starter}
